When cardinals determine the power set: inner models and H\"artig quantifier logic

We make use of some observations on the core model, for example assuming $V=L [ E ]$, and that there is no inner model with a Woodin cardinal, and $M$ is an inner model with the same cardinals as $V$, then $V=M$. We conclude in this latter situation that "$x=\mathcal{P} ( y )$" is $\Sigma_{1} ( Card )$ where $Card$ is a predicate true of just the infinite cardinals. It is known that this implies the validities of second order logic are reducible to $V_I$ the set of validities of the H\"artig quantifier logic. We draw some further conclusions on the L\"owenheim number, $\ell_{I}$ of the latter logic: that if no $L[E]$ model has a cardinal strong up to an $\aleph$-fixed point, and $\ell_{I}$ is less than the least weakly inaccessible $\delta$, then (i) $\ell_I$ is a limit of measurable cardinals of $K$; (ii) the Weak Covering Lemma holds at $\delta$.

==> pdwstyle.tex <==
%\documentclass{source}
%\usepackage[english]{babel}
%\usepackage{amsmath,amssymb,bbm}

%%%%%%%%%% Start TeXmacs macros
%\catcode`\<=\active \def<{
%\fontencoding{T1}\selectfont\symbol{60}\fontencoding{\encodingdefault}}
%\catcode`\>=\active \def>{
%\fontencoding{T1}\selectfont\symbol{62}\fontencoding{\encodingdefault}}
%\catcode`\|=\active \def|{
%\fontencoding{T1}\selectfont\symbol{124}\fontencoding{\encodingdefault}}
%\newcommand{\tmrsub}[1]{\ensuremath{_{\textrm{#1}}}}
%\newcommand{\tmstrong}[1]{\textbf{#1}}
%%%%%%%%%% End TeXmacs macros

\newcommand{\hi}{version Sep 23 15a)}
\newcommand{\abo}[2]{\ensuremath{#1 <_{\mathcal{O}}   #2}}
\newcommand{\calo}{ {\mathcal{O}}}
\newcommand{\calm}{\ensuremath{\mathcal{M}} }
\newcommand{\cali}{\ensuremath{\mathcal{I}} }
\newcommand{\calj}{{\mathcal{J}}}
\newcommand{\calk}{ {\mathcal{K}}}
\newcommand{\call}{ {\mathcal{L}}}
\newcommand{\calc}{C}
\newcommand{\gott}{\ensuremath{\mathfrak{T}}}
\newcommand{\GRP}{\ensuremath{(\ensuremath{\operatorname{GRP}}_{0} )}}
\newcommand{\LST}{\ensuremath{\call_{\dot{\in}}}}
\newcommand{\ent}{{{\em Entscheidungsproblem\/}}}
\newcommand{\bara}{\bar{{\alpha}}}
\newcommand{\bp}{\bar{{\pi}}}
\newcommand{\ts}{\ensuremath{T^{\ast}}}
\newcommand{\tsptwo}{\left.{\emp}\right) \
\ensuremath{_{\textrm{p\tmrsub{2}}}}}
\newcommand{\tptwo}{\ensuremath{T^{\ast} ( \varnothing )_{p_{2}}}}
\newcommand{\pe}{\ensuremath{P^{\ensuremath{\operatorname{\mathsf{eJ}}}}_{e}}}
\newcommand{\tmt}[1]{\ensuremath{\mathbbm{T}^{#1}}}
\newcommand{\p}[1]{\ensuremath{P^{\ensuremath{\operatorname{\mathsf{eJ}}}}_{#1}}}
\newcommand{\zx}[1]{\ensuremath{{^{#1}\zeta}}}
\newcommand{\Mx}[1]{\ensuremath{{^{#1} \!M}}}
\newcommand{\sx}[1]{\ensuremath{{^{#1} \Sigma}}}
\newcommand{\tx}[1]{\ensuremath{^{#1} T}}
\newcommand{\cst}{\ensuremath{\macro{C^{\ast}}}}
\newcommand{\tmcr}{\ensuremath{\curvearrowright}}
\newcommand{\cl}{\ensuremath{\curvearrowleft}}
\newcommand{\ou}{{\"o}}
\newcommand{\au}{{\"a}}
\newcommand{\uu}{{\"u}}
\newcommand{\go}{G{\"o}del}
\newcommand{\phiav}[1]{\ensuremath{\Phi^{\alpha}_{#1}}}
\newcommand{\phiaf}{\ensuremath{\Phi_{\ensuremath{\operatorname{fp}}}^{\alpha}}}
\newcommand{\phiabp}[2]{\ensuremath{\Phi_{\beta +1}^{(  \alpha )}}}
\newcommand{\phiab}[2]{\ensuremath{\Phi_{#2}^{#1}}}
\newcommand{\phivf}[1]{\ensuremath{\Phi_{\ensuremath{\operatorname{fv}}}^{#1}}}
\newcommand{\rar}{{\rightarrow}}
\newcommand{\midd}{ {\mid} }
\newcommand{\con}{{\hspace{-0.03em}\smallfrown \hspace{-0.03em}}}
\newcommand{\lt}{{\leq}\ensuremath{_{\textrm{T}}}}
\newcommand{\qu}{Q}
\newcommand{\pb}{\ensuremath{\Psi_{\beta}}}
\newcommand{\oy}{<\ensuremath{_{\textrm{y\tmrsub{0}}}}}
\newcommand{\oyr}{\ensuremath{>_{y_{0}}}}
\newcommand{\oye}{{\leq}\ensuremath{_{\textrm{y\tmrsub{0}}}}}
\newcommand{\ptwo}{{\mbox{{\em II\/}}}}
\newcommand{\pone}{{\mbox{{\em I\/}}}}
\newcommand{\uhr}{{\upharpoonright}}
\newcommand{\2}{{{\em II\/}}}
\newcommand{\1}{{{\em I\/}}}
\newcommand{\wff}{\ensuremath{\ensuremath{\operatorname{wff}}(y_{0} )}}
\newcommand{\nod}{{\noindent}}
\newcommand{\diam}{\ensuremath{}{\diamond}}
\newcommand{\lalp}{ {\pa{L\ensuremath{_{\textrm{{\alpha}}}},{\in}}}}
\newcommand{\cit}{{\macro{}{{\cite{\arg{k}}}}}}
\newcommand{\ul}{\ensuremath{\ulcorner}}
\newcommand{\ur}{\ensuremath{\urcorner}}
\newcommand{\cs}{\ensuremath{\ul \sigma \ur}}
\newcommand{\ct}{\ensuremath{\ul \tau \ur}}
\newcommand{\cso}{\ensuremath{\ul \sigma_{0} \ur}}
\newcommand{\co}[1]{\ensuremath{\ulcorner #1 \urcorner}}
\newcommand{\gp}[1]{\ensuremath{\prec #1 \succ}}
\newcommand{\tmfi}{\ensuremath{\ensuremath{\operatorname{Field}}( \prec )}}
\newcommand{\al}{\ensuremath{\aleph}}
\newcommand{\alo}{\ensuremath{\aleph_{\omega}}}
\newcommand{\cub}{c.u.b.}
\newcommand{\dff}{\ensuremath{\ensuremath{\operatorname{Def}}}}
\newcommand{\bu}{\ensuremath{\bullet } }
\newcommand{\nat}{\ensuremath{\mathbbm{N}}}
\newcommand{\re}{\ensuremath{\mathbbm{R}}}
\newcommand{\baire}{\ensuremath{\mathbbm{N}}\textsuperscript{\ensuremath{\mathbbm{N}}}}
\newcommand{\bai}{\textsuperscript{\ensuremath{\omega}}\ensuremath{\omega}}
\newcommand{\linf}{{\leq}\ensuremath{_{\textrm{{\infty}}}}}
\newcommand{\linfs}{<\ensuremath{_{\textrm{\text{{\tmstrong{\ensuremath{\infty}}}}}}}}
\newcommand{\leinf}{{\leq}\ensuremath{_{\textrm{\text{{\tmstrong{\ensuremath{\infty}}}}}}}}
\newcommand{\cant}{2\textsuperscript{\ensuremath{\mathbbm{N}}}}
\newcommand{\can}{\textsuperscript{\ensuremath{\omega}}2}
\newcommand{\rest}{{\upharpoonright}}
\newcommand{\emp}{{\varnothing}}
\newcommand{\pa}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\wst}{\ensuremath{S}}
\newcommand{\ws}[2]{\ensuremath{S}\textsuperscript{#1}\ensuremath{_{\textrm{#2}}}}
\newcommand{\wsone}[1]{\ensuremath{S}\textsuperscript{1}\ensuremath{_{\textrm{#1}}}}
\newcommand{\wstwo}[1]{\ensuremath{S}\textsuperscript{2}\ensuremath{_{\textrm{#1}}}}
\newcommand{\wthree}[1]{\ensuremath{S}\textsuperscript{3}\ensuremath{_{\textrm{#1}}}}
\newcommand{\es}[2]{\ensuremath{E}\textsuperscript{#1}\ensuremath{_{\textrm{#2}}}}
\newcommand{\esone}[1]{\ensuremath{E}\textsuperscript{1}\ensuremath{_{\textrm{#1}}}}
\newcommand{\estwo}[1]{\ensuremath{E}\textsuperscript{2}\ensuremath{_{\textrm{#1}}}}
\newcommand{\wet}{\ensuremath{E}}
\newcommand{\game}{\ensuremath{\Game}}
\newcommand{\games}{\ensuremath{\Game \Sigma^{0}_{3}}}
\newcommand{\szero}{\ensuremath{\Sigma^{0}_{3}}}
\newcommand{\hright}{{\hookrightarrow}}

\newcommand{\callt}{L\ensuremath{_{\textrm{T}}}}
\newcommand{\calt}{T}
\newcommand{\cald}{D}
\newcommand{\calu}{\ensuremath{\mathcal{U}}}
\newcommand{\lst}{\ensuremath{\mathcal{L}_{\dot{\in}}}}
\newcommand{\calw}{W}
\newcommand{\calv}{V}
\newcommand{\vp}{\ensuremath{\varphi}}
\newcommand{\om}[1]{\ensuremath{\omega_{1} ( #1 ) }}
\newcommand{\da}{{\downarrow}}
\newcommand{\ua}{{\uparrow}}
\newcommand{\la}{{\langle}}
\newcommand{\ra}{{\rangle}}
\newcommand{\ran}{\text{ran}}
\newcommand{\dom}{\text{dom}}
\newcommand{\back}{{\backslash}}
\newcommand{\power}{P}
\newcommand{\mar}{{\marginpar{\ensuremath{\rightarrow}}}}
\newcommand{\bm}{{\boldmath}}
\newcommand{\opistol}{\text{\ensuremath{O^{\pistol}}}}
\newcommand{\ie}{{\itshape{i.e.}}{\hspace{0.25em}}}
\newcommand{\eg}{{\itshape{e.g.}}{\hspace{0.25em}}}
\newcommand{\etc}{{\itshape{etc.}}{\hspace{0.25em}}}
\newcommand{\via}{{\itshape{via }}{\hspace{0.25em}}}
\newcommand{\cf}{{\itshape{cf. }}{\hspace{0.25em}}}
\newcommand{\mm}{{\itshape{m.m.}}{\hspace{0.25em}}}
\newcommand{\an}{{\wedge}}
\newcommand{\bigconj}{\ensuremath{\bigwedge \hspace{-1.0em} \bigwedge}}
\newcommand{\tmk}{\text{``}}
\newcommand{\proves}{{\vdash}}
\newcommand{\all}{{\forall}}
\newcommand{\Equi}{{\,\Longleftrightarrow\,}}
\newcommand{\equi}{{\,\longleftrightarrow\,}}
\newcommand{\ex}{{\exists}}
\newcommand{\Imp}{{\,\Rightarrow\,}}
\newcommand{\sset}{ {\, \subseteq  \,} }
\newcommand{\lr}{{\leftrightarrow}}
\newcommand{\imp}{{\,\longrightarrow\,}}
\newcommand{\ri}{{\,\rightarrow\,}}
%\newcommand{\nequiv}{{\not\equiv}}
\newcommand{\wt}{\tilde{\}}}
\newcommand{\finold}{\ensuremath{[ \alpha ]^{< \omega}}}
\newcommand{\rem}{{\noindent}{\bfseries{Remark: }}}
\newcommand{\fin}[1]{\ensuremath{[  ]^{< \omega}}}
\newcommand{\dlimtwo}{\ensuremath{\raisebox{-1.25\ensuremath{\operatorname{ex}}}{\overset{Lim}{\longrightarrow}
\hspace{0.25em}}}}
\newcommand{\dlim}{\text{{\raisebox{-1.25ex}{\ensuremath{\overset{Lim}{\longrightarrow}
\hspace{0.25em}}}}}}
\newcommand{\qed}{\hfill Q.E.D.}
\newcommand{\qedtwo}[1]{\hfill QED(#1)}
\newcommand{\pf}{{\noindent}{\textbf{Proof: }}}
\newcommand{\dfs}{\ensuremath{=_{\ensuremath{\operatorname{df}}}}}
\newcommand{\edfs}{\ensuremath{  \Equi_{\ensuremath{\operatorname{df}}}  }}
\newcommand{\pr}{\ensuremath{\prec}}
\newcommand{\pre}{\ensuremath{\preceq}}
\newcommand{\js}{\ensuremath{J_{s}}}
\newcommand{\jsb}{\ensuremath{J_{\bar{s}}}}
\newcommand{\jst}[3]{ \ensuremath{\langle J^{#1}_{#2} , #3 \rangle}}
\newcommand{\jnb}{J\ensuremath{_{\textrm{\bar{{\nu}}}}}}
\newcommand{\jn}{J\ensuremath{_{\textrm{{\nu}}}}}
\newcommand{\lam}[2]{\ensuremath{\Lambda ( #1 , #2 )}}
\newcommand{\nb}{\ensuremath{\bar{\nu}}}
\newcommand{\nbn}{\ensuremath{\bar{\nu} \prec \nu}}
\newcommand{\ns}{{\nu}\ensuremath{_{\textrm{s}}}}
\newcommand{\tmsb}{\ensuremath{\bar{s}}}
\newcommand{\nsb}{\ensuremath{\nu_{\bar{s}}}}
\newcommand{\maps}{\ensuremath{f: \bar{s} \Longrightarrow s}}
\newcommand{\mapnr}{\ensuremath{f \Longrightarrow \nu}}
\newcommand{\mapn}{\ensuremath{f: \bar{\nu} \Longrightarrow \nu}}
\newcommand{\mapg}[3]{\ensuremath{#1 : \overline{#2} \Longrightarrow #3}}
\newcommand{\onektuple}[1]{\ensuremath{#1_{1} , \ldots ,  #1_{k}}}
\newcommand{\zeroktuple}[1]{\ensuremath{#1_{0} , \ldots  , #1_{k}}}
\newcommand{\onentuple}[1]{\ensuremath{#1_{1} , \ldots  , #1_{n}}}
\newcommand{\zerontuple}[1]{\ensuremath{#1_{0} , \ldots  , #1_{n}}}
\newcommand{\ntuple}[2]{\ensuremath{#1_{1} , \ldots  , #1_{#2}}}
\newcommand{\otuple}[2]{\ensuremath{#1_{0} , \ldots  , #1_{#2}}}
\newcommand{\signk}{\ensuremath{\Sigma_{k}^{(n)}}}
\newcommand{\signo}{\ensuremath{\Sigma_{1}^{(n)}}}
\newcommand{\bsigno}{\ensuremath{\ensuremath{\boldsymbol{\Sigma}}_{1}^{(n)}}}
\newcommand{\bsigmo}{\ensuremath{\ensuremath{\boldsymbol{\Sigma}}_{1}^{(m)}}}
\newcommand{\sigmk}[1]{\ensuremath{\Sigma_{#1}^{(n)}}}
\newcommand{\sigmnk}[2]{\ensuremath{\Sigma_{#2}^{( #1 )}}}
\newcommand{\sigms}{ \ensuremath{\Sigma^{\ast}}}
\newcommand{\bsigms}{{\textbf{ \ensuremath{\Sigma^{\ast}}}}}
\newcommand{\lnn}{ \ensuremath{\Lambda (q, \nu )}}
\newcommand{\lns}{ \ensuremath{\Lambda (q,s)}}
\newcommand{\lnsp}{ \ensuremath{\Lambda^{+} (q,s)}}
\newcommand{\lnsl}{ \ensuremath{\Lambda (q,s| \lambda )}}
\newcommand{\fb}[1]{\ensuremath{\lambda (f_{( #1 ,q, \nu )} )}}
\newcommand{\fbb}[2]{\ensuremath{\lambda (f_{( #1 ,q,  #2 )} )}}
\newcommand{\fbs}[1]{\ensuremath{\lambda (f_{( #1 ,q,s)} )}}
\newcommand{\lis}{\ensuremath{l^{i}_{s}}}
\newcommand{\lhs}{\ensuremath{l^{i}_{\eta s}}}
\newcommand{\lls}{\ensuremath{l^{i}_{\lambda s}}}
\newcommand{\llf}{\ensuremath{\lambda = \lambda (f)}}
\newcommand{\csp}{C\ensuremath{_{\textrm{s}}}\textsuperscript{+}}
\newcommand{\csl}{C\ensuremath{_{\textrm{s|{\lambda}}}}}
\newcommand{\rn}{ \ensuremath{\rho^{n+1}_{M} > \kappa}}
\newcommand{\rhn}[1]{{\rho}\textsuperscript{#1}\ensuremath{_{\textrm{M}}}}
\newcommand{\rhnm}[2]{{\rho}\textsuperscript{#1}\ensuremath{_{\textrm{#2}}}}
\newcommand{\eqn}{{\omega}{\rho}\textsuperscript{n+1}\ensuremath{_{\textrm{M}}}{\leq}{\kappa}<{\omega}{\rho}\textsuperscript{n}\ensuremath{_{\textrm{M}}}}
\newcommand{\hnm}{H\textsuperscript{n}\ensuremath{_{\textrm{M}}}}
\newcommand{\oddpagetext}[1]{\newcommand{\pageoddheader}{{\small }}}
\newcommand{\evenpagetext}[1]{\newcommand{\pageevenheader}{{\small }}}

\def\pd{\mbox{$PD$\,}}
\def\ad{\mbox{$AD$\,}}

%\begin{document}


%\end{document}

